Instance-Guided Unsupervised Domain Adaptation for Robotic Semantic Segmentation

Semantic segmentation networks, which are essential for robotic perception, often suffer from performance degradation when the visual distribution of the deployment environment differs from that of the source dataset on which they were trained. Unsupervised Domain Adaptation (UDA) addresses this challenge by adapting the network to the robot's target environment without external supervision, leveraging the large amounts of data a robot might naturally collect during long-term operation. In such settings, UDA methods can exploit multi-view consistency across the environment's map to fine-tune the model in an unsupervised fashion and mitigate domain shift. However, these approaches remain sensitive to cross-view instance-level inconsistencies. In this work, we propose a method that starts from a volumetric 3D map to generate multi-view consistent pseudo-labels. We then refine these labels using the zero-shot instance segmentation capabilities of a foundation model, enforcing instance-level coherence. The refined annotations serve as supervision for self-supervised fine-tuning, enabling the robot to adapt its perception system at deployment time. Experiments on real-world data demonstrate that our approach consistently improves performance over state-of-the-art UDA baselines based on multi-view consistency, without requiring any ground-truth labels in the target domain.

==> contents/02-sota-Michele.tex <==
\section{Related Works}

\subsection{UDA Approaches for Semantic Segmentation}

Unsupervised domain adaptation (UDA) tackles the challenge of transferring the knowledge of a neural network from a source to a target domain under a strong assumption: no ground truth labels from the target domain are provided. This reflects the practical need of avoiding the costly and time--consuming manual annotation, which is particularly expensive for semantic segmentation, a task central in many in robotic scenarios~\cite{domain_adaptation_survey}.

A common approach for UDA is to use adversarial learning to align the distributions of the domains used to train and test the neural network at the levels of input data, intermediate features, and/or output predictions.

The pioneer work of~\cite{image_to_image_translation} presents a general paradigm based on unpaired image--to--image translation to align the embeddings extracted from different domains by the neural network. Each training example is converted into the other domain, thus generating fake images. Using them, the proposed method leverages adversarial learning and cycle consistency to build a latent space for the two domains in which feature distributions are domain invariant, and semantically similar images are projected into close vicinity. 
This paradigm is extended by CrDoCo~\cite{crdoco}. This framework combines massive image--to--image translation using GANs with adversarial learning and pixel--wise consistency. Its goal is to make the features extracted from an image and its restyled version indistinguishable, while ensuring that their predictions remain the same.

Instead of concentrating on inputs and inner features of the neural network, another promising solution is to perform adversarial learning on the output space of the neural network. The intuition is that the segmentation labels coming from different domains should be similar in terms of global layout and local context. Following this, the authors of~\cite{adapt_stuctured_output} propose to train a convolutional neural network to fool a discriminator tasked to disambiguate the domain from which its output masks are generated.
An extension of this approach is  ADVENT~\cite{advent_entropy}, a method that performs UDA leveraging the entropy of the predictions, calculated using the discrete pixel--wise distribution probability over object categories. Since the entropy tends to be low on the source domain but very high on data from the target domain, the authors propose an adversarial training scheme to make the target's entropy distribution similar to that of the source.

The limitations of the previous approaches come from the adversarial learning scheme, which is inherently unstable and, focusing only on domain confusion, completely ignores domain--specific cues. To overcome these, the more recent techniques for UDA leverage self--supervision with pseudo--labels inferred by the model itself from the target data. Since the inference on the target domain is inherently noisy and error--prone, the naive approach of treating the pseudo--labels as ground truths is impractical, as the adapted model will overfit on its misclassifications.

To solve this issue, a promising solution is to balance the influence of pseudo--labels during training, promoting high--confident predictions while penalizing noisy annotations. The work of~\cite{uncertanty_pseudo_labels} implements this paradigm by estimating the uncertainty of the predictions at a pixel level by computing the divergence between the outputs from two independent prediction layers. The uncertainty is then used as a regularization term during the fine--tuning to rectify the learning from noisy labels. An alternative approach is presented in~\cite{prototypical_labels_denoising}, where the weighting of pseudo--labels is calculated using the relative distance of the extracted features from their respective class centroid. The prototype for each object category is efficiently computed online during training (using moving average of the cluster centroids inside mini--batches) to avoid the early overfitting on noisy predictions. 

Another general approach for pseudo--labels refinement is the teacher--student framework: a student network, tasked to adapt to the target domain, is supervised by a teacher that, being gradually updated using exponential moving average (EMA) of the student, provides more stable and consistent pseudo--labels. Following this, the work in~\cite{class_balanced_self_training} rectifies the pseudo--labels using feature clustering on the target domain. A teacher network produces the embeddings for each pixel that are clustered together with a batch of randomly sampled features. The label of each pixel is updated based on the assigned cluster, thus providing more coherent and stable annotations that are used to supervise the student training. The authors of~\cite{mic} propose Masked Image Consistency (MIC), a technique in which the student is tasked to produce pseudo--labels on images in which random patches are masked. By doing this, the student (which is trained to be consistent with a teacher that access the unmasked data), learns to predict the class of missing portions using the global context of the image, improving generalization on the unseen domain. An extension of the teacher--student paradigm is presented in~\cite{revisiting_uda}. In this work, a student network is supervised by two teachers: the first one (updated with EMA) is applied to the outputs while the second, bigger teacher is fixed during training and provides transfer knowledge in the feature space.

\subsection{Leveraging Robot Embodiment for UDA}

Being typically tested for sim--to--real transfer in autonomous driving benchmarks, the aforementioned approaches operate in a single--frame manner, producing independent predictions for each image. This design completely neglects the unique settings of indoor mobile robots that, operating in high--cluttered human--centric environments,  are likely to observe the same portions of the scene multiple times. This peculiar behavior, specific to indoor robots deployments, can be effectively exploited to increase the quality of the pseudo--labels as the consistency of consecutive observations is useful to reduce the uncertainty and to improve the recognition of small, occluded, or partially visible objects.

The first work that leverages this idea is presented in~\cite{continual_adaptation_2d3d}, in which the authors introduce the concept of multi--view consistency. The intuition is simple: the model's predictions, being localized in the environment, should be consistent from multiple viewpoints. Following this, the method aggregates the single--frame 2D semantic predictions of the robot into a 3D voxel map, which stores the probability for each voxel to belong to a certain semantic class. This dense representation of the environment is then used for rendering pseudo--labels that aggregate information from multiple viewpoints, thus removing the intrinsic noise of the frame--by--frame model's predictions. This approach is extended in~\cite{informative_planning}, where the authors propose to leverage the robot embodiment for data acquisition in specific environmental locations. The idea is to aggregate in the dense environmental map not only the semantic labels, but also the uncertainty estimation of the model's predictions. In this way, the robot can collect novel views focusing on areas with high uncertainty to improve the quality of the 3D annotations. In the recent work of~\cite{uda_neural_rendering}, the voxel map is substituted with a semantic NeRF, a more compact spatial representation of the environment that allows the rendering of novel views (RGB images) and their respective pseudo--labels to augment the training data.

In this paper, we propose a step forward for multi--view consistency, which is not able to resolve the coherent misclassifications across multiple frames. To address this limitation, we integrate a zero--shot, instance--aware refinement step, which is applied after the rendering from the 3D map. It is specifically designed to assign a single semantic class to each object instance, a procedure that also removes the artifacts generated by the rendering procedure. Through extensive evaluation on real--world data, we demonstrate that fine--tuning with our improved pseudo--labels remarkably increases the performance of a neural network in unseen environments, without requiring ground--truth annotations. 


==> contents/images/figures/promts_differences.tex <==
\renewcommand{\imageone}{1020}
\renewcommand{\imagetwo}{0}
\renewcommand{\imagethree}{690}
\renewcommand{\imagefour}{409}



\renewcommand{\ww}{0.188\linewidth}

\begin{figure}[]
\centering
\begin{tabular}{@{}c@{ }c@{ }c@{ }c@{ }c@{ }}
{\small$\mathbf{Y}^\texttt{MC}$}& {\small$\mathbf{B}_\texttt{G}$ }& {\small$\mathbf{Y}^\texttt{IR}_\texttt{G}$ }&  {\small$\mathbf{B}_\texttt{I}$} & {\small $\mathbf{Y}^\texttt{IR}_\texttt{I}$} 
\\
\includegraphics[width=\ww]{contents/images/prompts_differences/\imageone/mc.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imageone/mask_grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imageone/grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imageone/mask_informed.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imageone/informed.png}
\\
\includegraphics[width=\ww]{contents/images/prompts_differences/\imagetwo/mc.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagetwo/mask_grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagetwo/grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagetwo/mask_informed.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagetwo/informed.png}
\\
\includegraphics[width=\ww]{contents/images/prompts_differences/\imagethree/mc.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagethree/mask_grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagethree/grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagethree/mask_informed.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagethree/informed.png}
\\

\includegraphics[width=\ww]{contents/images/prompts_differences/\imagefour/mc.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagefour/mask_grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagefour/grid.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagefour/mask_informed.png}
    &
    \includegraphics[width=\ww]{contents/images/prompts_differences/\imagefour/informed.png}
\\

\end{tabular}
    \caption{Comparison of the pseudo--labels obtained with our method using the \texttt{grid} ($\mathbf{Y}^\texttt{IR}_\texttt{G}$) and the \texttt{informed} ($\mathbf{Y}^\texttt{IR}_\texttt{I}$) prompt strategies, together with a representative object instance extracted by SAM ($\mathbf{B}_\texttt{G}$ and $\mathbf{B}_\texttt{I}$ for \texttt{grid} and \texttt{informed}, respectively). $\mathbf{I}^t$ and $\mathbf{Y}^\texttt{MC}$ indicates the multi--view consistent annotations. In the first two rows, the \texttt{grid} approach ensures better results, while in the last two we can see how guiding the prompts with \texttt{informed} increases the precision of the pseudo--labels.}
    \label{fig:promts_diff}
\end{figure}

==> contents/images/figures/pseudo_labels_5cm.tex <==
\renewcommand{\imageone}{5cm/grid/scene0005_00/64.png}
\renewcommand{\imagetwo}{5cm/grid/scene0004_00/570.png}
\renewcommand{\imagethree}{5cm/informed/scene0002_00/443.png}

\renewcommand{\imagefour}{5cm/informed/scene0003_00/632.png}

\renewcommand{\ww}{0.178\linewidth}

\begin{figure}[]
\begin{tabular}{@{}p{0.05cm}c@{ }c@{ }c@{ }c@{ }c@{ }}

& {\small$\mathbf{I}^t$} & {\small$\mathbf{Y}^*$ }& {\small$\mathbf{Y}^\texttt{MC}$ }&  {\small$\mathbf{Y}^\texttt{IR}$} & {\small $\mathbf{Y}^\texttt{GT}$} \\

\multirow{2}{*}{\rotatebox[origin=c]{90}{{\small\texttt{grid}}}}&
\includegraphics[trim=0 480 640 0, clip, width=\ww]{contents/images/pseudo_labels/\imageone}
    &
    \includegraphics[trim=0 0 640 480, clip,width=\ww]{contents/images/pseudo_labels/\imageone}
    &
    \includegraphics[trim=320 0 320 480, clip,width=\ww]{contents/images/pseudo_labels/\imageone}
    &
    \includegraphics[trim=640 0 0 480, clip,width=\ww]{contents/images/pseudo_labels/\imageone}
    &
    \includegraphics[trim=640 480 0 0, clip,width=\ww]{contents/images/pseudo_labels/\imageone}

 \\
&
 \includegraphics[trim=0 480 640 0, clip, width=\ww]{contents/images/pseudo_labels/\imagetwo}
    &
    \includegraphics[trim=0 0 640 480, clip,width=\ww]{contents/images/pseudo_labels/\imagetwo}
    &
    \includegraphics[trim=320 0 320 480, clip,width=\ww]{contents/images/pseudo_labels/\imagetwo}
    &
    \includegraphics[trim=640 0 0 480, clip,width=\ww]{contents/images/pseudo_labels/\imagetwo}
    &
    \includegraphics[trim=640 480 0 0, clip,width=\ww]{contents/images/pseudo_labels/\imagetwo}

 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{{\small\texttt{informed}\hspace{-0.4cm}}}}
 &
 \includegraphics[trim=0 480 640 0, clip, width=\ww]{contents/images/pseudo_labels/\imagethree}
    &
    \includegraphics[trim=0 0 640 480, clip,width=\ww]{contents/images/pseudo_labels/\imagethree}
    &
    \includegraphics[trim=320 0 320 480, clip,width=\ww]{contents/images/pseudo_labels/\imagethree}
    &
    \includegraphics[trim=640 0 0 480, clip,width=\ww]{contents/images/pseudo_labels/\imagethree}
    &
    \includegraphics[trim=640 480 0 0, clip,width=\ww]{contents/images/pseudo_labels/\imagethree}

 \\

 &
 \includegraphics[trim=0 480 640 0, clip, width=\ww]{contents/images/pseudo_labels/\imagefour}
    &
    \includegraphics[trim=0 0 640 480, clip,width=\ww]{contents/images/pseudo_labels/\imagefour}
    &
    \includegraphics[trim=320 0 320 480, clip,width=\ww]{contents/images/pseudo_labels/\imagefour}
    &
    \includegraphics[trim=640 0 0 480, clip,width=\ww]{contents/images/pseudo_labels/\imagefour}
    &
    \includegraphics[trim=640 480 0 0, clip,width=\ww]{contents/images/pseudo_labels/\imagefour}

 \\
 
 
\end{tabular}
    \caption{Examples of the instance--aware pseudo--labels generated by our method ($\mathbf{Y}^\texttt{IR}$) obtained with the \texttt{grid} (top) and \texttt{informed} (bottom) strategies compared with the multi--view consistent ($\mathbf{Y}^\texttt{MC}$) and the raw ($\mathbf{Y}^*$) annotations. $\mathbf{Y}^t$ and $\mathbf{Y}^\texttt{GT}$ are, respectively, the RGB images and their relative ground--truth segmentations. }
    \label{fig:pseudo_labels_5cm}
\end{figure}

==> contents/images/labels_colors.tex <==
\begin{table*}[]

\centering

\begin{tabular}{lllllll}
\toprule

\classwall&\classfloor&\classcabinet&\classbed&\classchair&\classsofa&\classtable\\
\classdoor&
\classwindow&\classbookshelf&\classpicture&\classcounter&\classblinds&\classdesk\\
\classshelves&
\classcurtain&\classdresser&\classpillow&\classmirror&\classfloormat&\classclothes\\
\classceiling&
\classbooks&\classrefrigerator&\classtelevision&\classpaper&\classtowel&\classshowercurtain\\
\classbox&
\classwhiteboard&\classperson&\classnightstand&\classtoilet&\classsink&\classlamp\\
\classbathtub&
\classbag&\classotherstructure&\classotherfurniture&\classotherprop&&\\
\bottomrule
\end{tabular}
    \caption{Color code of labels}\label{tab:labels_colors}

\end{table*}



==> contents/tables/test_20.tex <==
\setlength{\tabcolsep}{0.5em}
\begin{table}[]
\scriptsize
\centering

\begin{tabular}{c|ccc|cccc}
\toprule
&\multicolumn{3}{c|}{Baselines} & \multicolumn{4}{c}{Our method}\\
Scene & PT & VC~\cite{continual_adaptation_2d3d}& $\Delta_{\text{PT--VC}}$ &IR$_{I}$ & $\Delta_{\text{VC--IR}_{I}} $& IR$_{G}$ & $\Delta_{\text{VC--IR}_{G}} $\\
\midrule
 1 & 44,1&	48,2&	9,3\%&	    49,3&	2,3\%&	   51&	5,8\%\\	
 2	& 36,2&	31,3&	-13,5\%&	34,4&	9,9\%&	   33,6&	7,3\%\\	
 3	& 22,9&	21	&   -8,3\%&		23,2&	10,5\%&	  21,4&	1,9\%\\	
 4	& 50,2&	51,1&	1,8	\%&	    52,5&	2,7\%&	  52,5&	2,7\%\\	
 5	& 39,5&	40,1&	1,5	\%&	    44,4&	10,7\%&	 44,5&  11,0\%\\	
 6	& 35&	31,9&	-8,9\%&		34,1&	6,9\%&	 33,9&	6,3\%\\	
 7	& 56,7&	63,5&	12,0\%&		63,5&	0,0\%&	60,7&	-4,4\%\\	
 8	& 29,5&	25,1&	-14,9\%&	26,3&	4,8\%&		   25,2&	0,4\%\\	
 9	& 55,9&	65,3&	16,8\%&		69&  	5,7\%&		   70,2&	7,5\%\\	
 10&73,3&	71,9&	-1,9\%&		74,7&	3,9\%&		   75,3&	4,7\%\\	\midrule
Avg	 &   44,3&	44,9&	-0,6\%&		47,1&	5,7\%&		   46,8&	4,3\%\\

\bottomrule
\end{tabular}
\caption{Improvements of the models tested on the last 20\% of the sequence (voxel 5cm).}\label{tab:data_quantity}
\vspace{-0.5cm}

\end{table}

==> contents/tables/test_all.tex <==
\setlength{\tabcolsep}{0.43em}
\begin{table*}[t]
\scriptsize
\centering

\begin{tabular}{c|c|cc|cccccc||c|cc|cccccc}
\toprule
\multicolumn{19}{c}{Training and testing inside the same sequence: the first 80\% is used for fine-tuninin, the last 20\% for testing}\\\midrule
&&\multicolumn{2}{c|}{Baseline (5cm)} & \multicolumn{6}{c||}{Our method}&&\multicolumn{2}{c|}{Baseline (3cm)} & \multicolumn{6}{c}{Our method}\\
Env & \PT & \MC& $\Delta_{\text{\PT}}$ &\IRG & $\Delta_{\text{\MC}} $& \IRI & $\Delta_{\text{\MC}} $ & \IRGI & $\Delta_{\text{\MC}} $& \PT& \MC& $\Delta_{\text{\PT}}$ &\IRG & $\Delta_{\text{\MC}} $& \IRI & $\Delta_{\text{\MC}} $ & \IRGI & $\Delta_{\text{\MC}} $ \\
\midrule
 
 1	&    44,2&	48,2&	9,0\%&	    \bestvalue{51}&	    5,8\%&	   49,3&	  2,3\%& \secondvalue{50,9} & 5,6\% &	  44,2&	47,6&	7,7\%&	    50,1&	5,3\%&	    \secondvalue{50,4}&	5,9\% &\bestvalue{51}	&7,1\%\\[0.05cm]
 2	 &   \bestvalue{36,2}&	31,3&	-13,5\%&	33,6&	7,3\%&	   34,4&	  9,9\%&	\secondvalue{34,8} &	11,2\% &    \bestvalue{36,2}&	34,4&	-5,0\%&	    34,5&	0,3\%&	    \secondvalue{34,9}&	1,5\% &33,8&	-1,7\%\\[0.05cm]
 3	&    22,9&	21&	    -8,3\%&	    21,4&	1,9\%&	   \bestvalue{23,2}&	  10,5\%&	\secondvalue{22,9}&	9,0\%  &   22,9&	21,7&	-5,2\%&	    22,6&	4,1\%&	    \secondvalue{23,1}&	6,5\%&\bestvalue{23,2}	&6,9\%\\[0.05cm]
 4&	 50,1&	51,1&	2,0\%&	    52,5&	2,7\%&	   \secondvalue{52,5}&	  2,7\%&	\bestvalue{53,4}&	4,5\% &    50,1&	52,4&	4,6\%&	    \secondvalue{52,9}&	1,0\%&	    49,5&	-5,5\%&\bestvalue{53,7}	&2,5\%\\[0.05cm]
 5&	 39,7&	40,1&	1,0\%&	    \secondvalue{44,5}&	11,0\%&	   44,4&      10,7\%&	 \bestvalue{44,7}&	11,5\%  &   39,7&	45&	    13,4\%&	    \secondvalue{47,2}&	4,9\%&	    46,1&	2,4\%&\bestvalue{47,3}&	5,1\%\\[0.05cm]
 6&	 \bestvalue{35}&    31,9&	-8,9\%&	    33,9&	6,3\%&	   34,1&      6,9\%&	\secondvalue{34,9}&	9,4\% &    35&	    33,5&	-4,3\%&	    \secondvalue{39,5}&	17,9\%&	    38,8&	15,8\%&\bestvalue{40,1}&	19,7\%\\[0.05cm]
 7&	 56,7&	\secondvalue{63,5}&	12,0\%&	    60,7&	-4,4\%&	   \bestvalue{63,5}&      0,0\%&	60,9&	-4,1\% &    56,7&	\bestvalue{63}&	    11,1\%&	    \secondvalue{60,9}&	-3,3\%&	    56,7&	-10,0\%&59,5&	-5,6\%\\[0.05cm]
 8&	  \bestvalue{29,5}&	25,1&	-14,9\%&	25,2&	0,4\%&	   26,3&      4,8\%&	\secondvalue{27,6} &	10,0\%  &    \bestvalue{29,5}&	25,1&	-14,9\%&	24,1&	-4,0\%&	    \secondvalue{27}&	   7,6\%&25,7&	2,4\%\\[0.05cm]
 9	&    55,9&	65,3&	16,8\%&	    \bestvalue{70,2}&	7,5\%&     69&  	  5,7\%&	\secondvalue{69,2}&	6,0\% &    55,9&	66,9&	19,7\%&	    \bestvalue{70,9}&	6,0\%&	    69,8&	4,3\%&\secondvalue{69,9}	&4,5\%\\[0.05cm]
 10&	73,4&	71,9&	-2,0\%&	    \bestvalue{75,3}&	4,7\%&     74,7&      3,9\%&	 \secondvalue{75}&	4,3\% &   73,4&	73,2&	-0,3\%&	    \bestvalue{75,7}&	3,4\%&	    \secondvalue{75,6}&	3,3\%&75,3&	2,9\%\\\midrule
Avg&	     44,4&	44,9&	-0,7\%&	    46,8&	4,3\%&	 \secondvalue{46,8}&      5,7\%&	\bestvalue{47,4}&	6,7\% &    44,4&	46,3&	2,7\%&	    \secondvalue{47,8}&	3,6\%&	    47,2&	3,2\%&\bestvalue{48,0}&	4,4\%\\\bottomrule
\toprule
\multicolumn{19}{c}{Training and testing in two different sequences of the same environment}\\\midrule
&&\multicolumn{2}{c|}{Baseline (5cm)} & \multicolumn{6}{c||}{Our method}&&\multicolumn{2}{c|}{Baseline (3cm)} & \multicolumn{6}{c}{Our method}\\
Env & \PT & \MC& $\Delta_{\text{\PT}}$ &\IRG & $\Delta_{\text{\MC}} $& \IRI & $\Delta_{\text{\MC}} $ & \IRGI & $\Delta_{\text{\MC}} $& \PT& \MC& $\Delta_{\text{\PT}}$ &\IRG & $\Delta_{\text{\MC}} $& \IRI & $\Delta_{\text{\MC}} $ & \IRGI & $\Delta_{\text{\MC}} $ \\
\midrule
1&	47,1&	49,6&	5,3\%&      \bestvalue{55}&	    10,9\%&	51,2&	3,2\%& \secondvalue{54,3}&	9,5\%	& 47,1&	48,9&	3,8\%&	    \secondvalue{50,6}&	3,5\%&	    49,5&	1,2\% &\bestvalue{50,8}	&3,9\%\\[0.05cm]
2&	\bestvalue{44,1}&	35,2&	-20,2\%&    39,6&	12,5\%&	\secondvalue{39,6}&	12,5\%& 39,3&	11,6\%&	 \bestvalue{44,1}&	\secondvalue{42,1}&	-4,5\%&	    41,8&	-0,7\%&	      41,6&	-1,2\%&41,6 &	-1,2\%\\[0.05cm]
3&	30,6&	30,5&	-0,3\%&	    32,8&	7,5\%&   \secondvalue{34,4}&	12,8\%&	  \bestvalue{34,7} &	13,8\%& 30,6&	31,5&	2,9\%&	    \bestvalue{36,5}&	15,9\%&	     35,1&	11,4\%&\secondvalue{36,3}&	15,2\%\\[0.05cm]
4&	55,3&	55,8&	0,9\%&      \secondvalue{57,2}&	2,5\%&   56,2&	0,7\%& \bestvalue{57,7}	&3,4\%&    55,3&	57,1&	3,3\%&	    \bestvalue{57,4}&	0,5\%&	    56,8&	-0,5\%&\secondvalue{57,2}&	0,2\%\\[0.05cm]
6&	49,2&	50,5&	2,6\%&	   52,8&	4,6\%&  \bestvalue{54,7}&	8,3\%& \secondvalue{53}&	5,0\%&   49,2&	51,2&	4,1\%&	    54,8&	7,0\%&	    \bestvalue{55,8}&	9,0\%&\secondvalue{54,8}	&7,0\%\\[0.05cm]
7&	52&	54,4&	4,6\%&	55,5&	2\%&	\bestvalue{57,2}&	    5,1\%& \secondvalue{56,2}	&3,3\%&   52&	54,1&	4\%&54,8&	1,3\%&	    \secondvalue{55,1}&	1,8\%&\bestvalue{55,3}&	2,2\%\\[0.05cm]
10&	57,5&	63,2&	9,9\%&	    \secondvalue{68,7}&	8,7\%&  67,6&	7,0\%& \bestvalue{68,7}&	8,7\%&   57,5&	65,2&	13,4\%&	    \secondvalue{69,1}&	6,0\%&	    68,3&	4,8\%&\bestvalue{70,1}&	7,5\%\\\midrule
Avg&48&	48,5&	0,4\%&	    \secondvalue{51,7}&	7\%&  51,6&	7,1\%&  \bestvalue{52,0}&	7,9\%&  48&	50&	3,9	\%&    \secondvalue{52,1}&	4,8	\%&    51,7&	3,8\%&\bestvalue{52,3}	&5,0\%\\

\bottomrule


\end{tabular}
\caption{Improvements of $f_{\theta_t}^{seg}$ trained using the instance--aware pseudo--labels using \texttt{grid} (\IRG), \texttt{informed} (\IRI), and the combination (\IRGI) of the strategies compared with the fine--tuning using the multi--view consistent annotations (\MC) and the outputs of the pre--trained model $f_{\theta_s}^{seg}$ (\PT). The voxel size is set to 5cm and 3cm. Training and testing is performed using the first 80\% and the last 20\% of the first sequence of each environment. Best and second best performances are in \bestvalue{bold} and \secondvalue{underlined}.}
\label{tab:performance_20}
\vspace{-0.5cm}

\end{table*}

==> contents/tables/test_new_sequence.tex <==
\setlength{\tabcolsep}{0.5em}
\begin{table}[]
\scriptsize
\centering

\begin{tabular}{c|ccc|cccc}
\toprule
&\multicolumn{3}{c|}{Baselines} & \multicolumn{4}{c}{Our method}\\
Scene & PT & VC~\cite{continual_adaptation_2d3d}& $\Delta_{\text{PT--VC}}$ &IR$_{I}$ & $\Delta_{\text{VC--IR}_{I}} $& IR$_{G}$ & $\Delta_{\text{VC--IR}_{G}} $\\
\midrule
1&	47,1&	49,6&	5,3\%&	51,2&	3,2\%&	55&	10,9\%\\
2&	44,1&	35,2&	-20,2\%&	39,6&	12,5\%&	39,6&	12,5\%\\
3&	30,6&	30,5&	-0,3\%&	34,4&	12,8\%&	32,8&	7,5\%\\
4&	55,3&	55,8&	0,9\%&	56,2&	0,7\%&	57,2&	2,5\%\\
6&	49,2&	50,5&	2,6\%&	54,7&	8,3\%&	52,8&	4,6\%\\
7&	49,2&	43,3&	-12,0\%&	45&	3,9\%&	42,3&	-2,3\%\\
10&	57,5&	63,2&	9,9\%&	67,6&	7,0\%&	68,7&	8,7\%\\\midrule
Avg&	47,6&	46,9&	-2,0\%&	49,8&	6,9\%&	49,8&	6,3\%\\

\bottomrule
\end{tabular}
\caption{Improvements of the models trained and tested in different sequences of the same scene. Voxel size 5cm.}\label{tab:data_quantity}
\vspace{-0.5cm}

\end{table}
